The Consistency of Probabilistic Databases with Independent Cells

A probabilistic database with attribute-level uncertainty consists of relations where cells of some attributes may hold probability distributions rather than deterministic content. Such databases arise, implicitly or explicitly, in the context of noisy operations such as missing data imputation, where we automatically fill in missing values, column prediction, where we predict unknown attributes, and database cleaning (and repairing), where we replace the original values due to detected errors or violation of integrity constraints. We study the computational complexity of problems that regard the selection of cell values in the presence of integrity constraints. More precisely, we focus on functional dependencies and study three problems: (1) deciding whether the constraints can be satisfied by any choice of values, (2) finding a most probable such choice, and (3) calculating the probability of satisfying the constraints. The data complexity of these problems is determined by the combination of the set of functional dependencies and the collection of uncertain attributes. We give full classifications into tractable and intractable complexities for several classes of constraints, including a single dependency, matching constraints, and unary functional dependencies.

==> beyond.tex <==
\section{Beyond Unary  Dependencies}\label{sec:beyond-unary}
We leave open the question of whether and how the classification of Theorem~\ref{thm:unary:trichotomy} can be extended to general sets of FDs. In this section, we discuss simple special cases of non-unary FDs where we can generalize the unary case rather directly. For example, the previous machinery can easily cover the simplest case of a singleton set $\set{X\ra Y}$. 
\begin{theorem}\label{thm:one-FD}
Let $X\ra Y$ be an FD and $R$ a schema that contains $X\cup Y$. Assume, without loss of generality, that $X\cap Y=\emptyset$. If $X$ consists of only certain attributes, then all three problems are solvable in polynomial time. Otherwise, imputability is NP-complete and the probability of consistency is $\fpsharpp$-complete.
\end{theorem}
\begin{proof}
The tractability side follows from Theorem~\ref{thm:lhs-certain-poly}.
The hardness side is due to straightforward reduction from $\uca A\ra B$.
\end{proof}

We now discuss FD sets of form $X\lra Y$. We refer to a constraint of this form as a \e{matching constraint} like it is sometimes referred to in the literature (e.g.,~\cite{DBLP:conf/icdt/CarmeliGKLT21}). We restrict the discussion to the problem of finding a most probable imputation. The complexity of the other two problems remains open for future research. 
To cover the general case, we begin with some lemmas. We will prove the following. 

\begin{theorem}\label{thm:matching-dichotomy}
Let $X\lra Y$ be a matching constraint such that $X\not\subseteq Y$ and $Y\not\subseteq X$, and at least one attribute in $X\cup Y$ is uncertain. 
\begin{enumerate}
    \item If either $X$ or $Y$ consists of only certain attributes, then a most probable imputation can be found in polynomial time. In any other case, it is NP-hard to find a most probable imputation. 
    \item The probability of consistency is $\fpsharpp$-hard.
\end{enumerate}

\end{theorem}

Next, we prove Theorem~\ref{thm:matching-dichotomy}. We begin with the tractability.

\begin{lemma}\label{lemma:matching-certainside-tractable}
Let $X\lra Y$ be a matching constraint such that either $X$ or $Y$ consists of only certain attributes. A most probable imputation can be found in polynomial time.
\end{lemma}
\begin{proof}
We show a reduction to the case of $A\lra\tB$, which is tractable due to Proposition~\ref{prop:A_lra_tildeB_poly}. Without loss of generality, suppose that all attributes of $X$ are certain, and all attributes of $Y$ are uncertain. Given an input $U$ for $X\lra Y$, we construct an instance $U_0$ for  $A\lra\tB$ with $\tids(U_0)=\tids(U)$ by converting over tuple of $U$ into a tuple of $U_0$. The construction is simple: for each identifier $i\in\tids(U)$, the tuple
$U_0[i]$ is obtained as follows:
\begin{itemize}
    \item $U_0[i](A)=\pi_X U[i]$;
    \item $U_0[i](B)$ is the distribution over all possible tuples that can be generated from
    $\pi_Y U[i]$, each with its probability (i.e., the product of the values of the different attributes of $Y$).
\end{itemize}
The correctness of the reduction is straightforward. 
\end{proof}

We will need the following lemma.

\begin{lemma}\label{lemma:atb-lra-tbc}
For $A\tB\lra\tB C$, it is NP-hard to find a most probable imputation.
\end{lemma}
\begin{proof}
We show a reduction from the problem of 
\e{maximum edge covering by triangles}, which is the following problem: given a tripartite graph $(V_1\dot\cup V_2\dot\cup V_3,E)$, find the maximum number of edge-disjoint triangles. Given an instance for this problem, we construct a CIR $U$ as follows. 

For every edge $\set{a,c}$ between $V_1$ and $V_3$, let
$x_{\set{a,c}}$ be a fresh new constant, and let $V_{a,c}$ be the set of all vertices $b\in V_2$ such that $\set{a,b,c}$ is a triangle. We assume that $V_{a,c}$ is nonempty, or otherwise we can ignore $\set{a,c}$ in our problem.
Let $\epsilon$ be the number $\frac{1}{|V_2|^2+1}$. 
We define the distribution 
$\delta_{a,c}$ to be the one over $\set{x_{a,c}}\cup V_{a,c}$ given by $\delta_{a,c}(x_{a,c})\defeq\epsilon$ and
$\delta_{a,c}(b)\defeq(1-\epsilon)/|V_{a,c}|$ otherwise. Then, for each edge $\set{a,c}$ between $V_1$ and $V_3$ we have in $U$ the tuple $(a,\delta_{a,c},c)$. 

Note that $U$ is imputable: an imputation can be produced by selecting $\set{x_{a,c}}$ for each $\delta_{a,c}$. 
We claim that from a most-probable imputation $r$ for $U$ we can easily obtain a maximum number of edge-disjoint triangles. The construction is straightforward: we take every triangle
$(v_1,v_2,v_3)$ that forms a tuple of $r$. To see that it is indeed a collection of edge-disjoint triangles, observe that no two distinct tuples 
of $r$ have can have the same $v_1$ and $v_3$ since this is how  $U$ is constructed; similarly, no two distinct tuples of $r$ can have the same $v_1$ and $v_2$ (due to $A\tB\ra C$) or the same  $v_2$ and $v_3$ (due to $C\tB\ra A$).

Finally, we need to show that a most probable imputation indeed induces a set of triangles of a maximal size. This is true due to the choice of $\epsilon$---any imputation with $\ell+1$ tuples with 
$\set{x_{a,c}}$ values has a lower probability than any imputation with $\ell$ tuples with 
$\set{x_{a,c}}$ values. This completes the proof.
\end{proof}

We can now prove Theorem~\ref{thm:matching-dichotomy}.
\begin{proof}[Proof of Theorem~\ref{thm:matching-dichotomy}]
The tractability side of Part~1 is proved in Lemma~\ref{lemma:matching-certainside-tractable}. The hardness side of both parts is proved as follows. If $X$ and $Y$ share an uncertain attribute $\tB$, then we can easily devise a reduction from $A\tB\lra\tB C$, where we establish hardness in Lemma~\ref{lemma:atb-lra-tbc}. Otherwise, there are attributes $\tA$ in $X$ and $\tB$ in $Y$ such that $\tA\neq\tB$. Then we can easily devise a reduction from
$\tA\lra\tB$, where hardness is established in Lemma~\ref{lemma:hardness-tildeA-lra-tildeB}. 

\benny{Not done with the \#P-hardness part...}
\end{proof}


==> intro.tex <==

\section{Introduction}\label{sec:intro}

\eat{
\begin{figure}[!htb]
\centering
    \begin{subfigure}[b]{0.4\textwidth}
     \centering
    \begin{enumerate}
        \item $specialist?,time \rightarrow room$ 
        \item $room,time \rightarrow specialist?$
    \end{enumerate}
    \vspace{-3mm}
    \caption{Functional Dependencies.}\label{fig:fds-poly}
    \end{subfigure}
    \caption{Most probable imputation with FD (1) (NP-Hard): $t_1$[specialist] = Dr. Bart, $t_1$[specialist] = Dr. Lisa, and $t_1$[specialist] = Dr. Maggie with probability 14.4\%. Most probable imputation with FDs (1) and (2) (PTIME): $t_1$[specialist] = Dr. Bart, $t_1$[specialist] = Dr. Lisa, and $t_1$[specialist] = Dr. Bart  with probability 9.6\%.}\label{fig:ex-hard}
\end{figure}
}




Various database tasks amount to reasoning about relations where attribute values are uncertain. To name a few, systems for \e{data cleaning} may detect errors and suggest alternative fixes with different confidence scores~\cite{RekatsinasCIR17,DBLP:conf/icdt/SaIKRR19,DBLP:conf/sigmod/HeidariMIR19}, approaches to \e{data repairs} may suggest alternative values due to the violation of integrity constraints (e.g., key constraints and more general functional dependencies)~\cite{AndritsosFM06,DBLP:journals/tods/Wijsen05}, and algorithms for \e{missing-data imputation} may suggest a probability distribution over possible completions of missing values~\cite{DBLP:journals/jmlr/BiessmannRSNSTL19,DBLP:conf/sigmod/MayfieldNP10}.
Such uncertainty is captured as a probabilistic database in the
so called \e{attribute-level uncertainty}~\cite{DBLP:series/synthesis/2011Suciu} (as opposed to the commonly studied \e{tuple-level uncertainty}~\cite{DBLP:conf/vldb/DalviS04}). 

In this paper, we refer to a relation of a probabilistic database in the attribute-level uncertainty as a Cell-Independent Relation (CIR). 
A CIR is a probabilistic database with a single relation, where the content of a cell is a distribution over possible values, and moreover, different cells are probabilistically independent. 
The CIR is the correspondent of a relation in the \e{Tuple-Independent Database} (TID)  under the \e{tuple-level uncertainty}, where the existence of each tuple is uncertain (while its content is certain), and different tuples are probabilistically independent~\cite{DBLP:series/synthesis/2011Suciu}. (In contrast, the tuples of a CIR always exist, but their content is uncertain.) 

For example, Figure~\ref{fig:specialist-cir} shows a CIR where we have uncertain information about specialists attending rooms (e.g., since their attendance is determined by noisy sensors). Figure~\ref{fig:spokesperson-cir} depicts an example of a CIR that stores businesses along with their spokespeople and headquarters locations (inspired by King of the Hill \ag{Not sure if needed}); some information is noisy (e.g., since the rows are scraped from Web pages), and particularly the identity of the spokesperson and the business location. Some attributes (here $\att{room}$ and $\att{business}$) are certain and have deterministic values. The uncertain attributes (e.g., $\uca{\att{specialist}}$) are marked by a question mark. We later explain how this distinction has crucial impact on the complexity of CIRs.

%The database contains a tuple for each of the websites. Probabilities are assigned to the different options, based on the strength of the association between the business and the spokesperson/location on a particular website. For example, in one website, represented by the second tuple, the business Mega Lo Mart has a 0.45 association with Mangione as their spokesperson and 0.5 association with Thatherton. In another website, represented by the third tuple, Mega Lo Mart has a 0.4 association with Mangione as their spokesperson and 0.6 association with Buckley.


We study inference problems over CIRs with respect to underlying integrity constraints \ag{This comes a bit out of the blue. Maybe preface this by saying that it makes sense to consider the consistency w.r.t constraints and not just fill in the most probable values?}. 
By a \e{consistent sample} we refer to a possible world of the CIR that has a nonzero probability and that satisfies the integrity constraints. 
We investigate the computational complexity of consistency tasks where the underlying integrity constraints are formed as Functional Dependencies (FDs). The first task is what is known as finding a \e{most probable database} (studied for tuple-level uncertainty~\cite{GVSBUDA14,DBLP:journals/tods/LivshitsKR20} as ``MPD''), that is, a consistent sample with a maximal probability. To this end, we need to be able to solve the \e{possible consistency} problem: determine whether a consistent sample exists at all, or equivalently, whether the given CIR satisfies the constraints with a nonzero probability.

We also study the task of calculating the above probability exactly (beyond just deciding whether it is nonzero), that is, the probability that (a random sample of) the given CIR satisfies the underlying functional dependencies. 
This analysis is interesting not only for shedding light on the possible consistency problem. As we explain in Section~\ref{sec:problems}, computing this probability is useful to any type of constraints over CIRs, as the tractablity of this probability implies that we can efficiently sample uniformly  from the conditional space. 


Our study adopts the standard yardstick of \e{data complexity}~\cite{DBLP:conf/stoc/Vardi82}, where we fix the relational schema and the set of functional dependencies. The schema mentions not only what attributes are in the header of the relation, but also \e{which attribute is certain and which attribute is uncertain}. The complexity of the problems can be different for different combinations of schema and constraints, and we aim for a detailed understanding of which combinations are tractable and which are not.
\ag{I think the problems that we study are a bit scattered here. Maybe first state all three and then explain each one?}

In contrast to the state of affairs in the attribute-level uncertainty, for \e{tuple-level uncertainty}  much more is known about MPD (i.e., finding the most likely instance of a probabilistic database conditioned on conformance to a set of FDs). In the case of tuple-independent databases, 
Gribkoff, Van den Broeck, and Suciu~\cite{GVSBUDA14} established dichotomy in the complexity of MPD for sets of unary FDs. This dichotomy has been generalized by Livshits, Kimelfeld and Roy~\cite{DBLP:journals/tods/LivshitsKR20} to a full classification over all sets of FDs, where they also established that the problem is equivalent to finding a \e{cardinality repair} of an inconsistent database. Carmeli et al.~\cite{DBLP:conf/icdt/CarmeliGKLT21} showed that two tractable cases, namely a \e{single FD} and a \e{matching constraint}, remain tractable even if the FDs are treated as \e{soft constraints} (where every violation incurs a cost). 
In this work, we aim to bring our understanding of attribute-level uncertainty closer to  tuple-level uncertainty.

\subparagraph*{Results.}
We establish classification results on several classes of functional dependencies: singleton FDs, matching constraints (i.e., FD sets of the form $\set{X\ra Y,Y\ra X}$), and arbitrary sets of unary FDs. Each classification consists of three internal classifications---one for each of the three problems we study (possible consistency, most probable database, and the probability of consistency). In every case, finding a most probable database is tractable whenever possible consistency is tractable. There are cases where the probability of consistency is intractable in contrast to the tractability of the most probable database, but we did not find any case where the other direction holds (and we will be surprised if such case exists). 
We also establish some general conclusions beyond these classes. For example, in Theorem~\ref{thm:all-uncertain-all-hard} (of Section~\ref{sec:single-matching}) we claim that if we make no assumption 
that some attributes are certain, then possible consistency is hard for \e{every nontrivial set of FDs}.

\subparagraph*{Related work.}

A most probable database is the same as the ``Most Likely Intention'' (MLI) in the framework of Probabilistic Unclean Databases (PUD) of De Sa et al.~\cite{DBLP:conf/icdt/SaIKRR19}, in the special case where the \e{intention model} demands hard constraints and the \e{realization model} applies random changes to cells independently in what they refer to as \e{parfactor/update} PUD. They showed that finding an MLI of a parfactor/update PUD generalizes the problem of finding an \e{update repair} of an inconsistent database with a minimum number of value changes.
In turn, finding a minimal update repair has been studied in the literature and several complexity results are known for special cases of FDs, such as hardness (e.g., for the FD set $\set{A\ra B,B\ra C}$ due to Kolahi and Lakshmanan~\cite{DBLP:conf/icdt/KolahiL09}) and tractability (e.g., for lhs-chains such as $\set{A\ra B, AD\ra C}$ due to Livshits et al.~\cite{DBLP:journals/tods/LivshitsKR20}). There are, though, substantial differences between finding a most probable consistent sample of a CIR and finding an optimal update repair of an inconsistent database, at least in the variations where complexity results are known. First, they allow to select \e{any} value (from an infinite domain) for a cell, in contrast to the distributions of the CIR that can limit the space of allowed values; indeed, this plays a major role in past repair algorithms (e.g., Proposition 5.6 of~\cite{DBLP:journals/tods/LivshitsKR20} and Algorithm \textsc{FindVRepair} of~\cite{DBLP:conf/icdt/KolahiL09}). Second, they allow to change the value of \e{any} attribute and do not distinguish between uncertain attributes (where changes are allowed) and certain ones, as we do here; this is critical since, again, without such assumptions the problem is intractable for every nontrivial set of FDs (Theorem~\ref{thm:all-uncertain-all-hard}).

The problem of possible consistency does not have a nontrivial correspondence in the tuple-independent database model since, there, if there is any consistent sample then the subset that consists of all deterministic tuples (i.e., ones with probability one) is such a sample. The probability of consistency might be reminiscent of the problem of \e{repair counting} that was studied for subset repairs~\cite{DBLP:journals/jcss/LivshitsKW21,DBLP:conf/pods/CalauttiLPS22a}. Besides the fact that subset repairs are about tuple-level uncertainty (and no probabilities are involved), here we do not have any notion of \e{maximality} (while a repair is required to be a maximal consistent subset).

A CIR can be easily translated into a relation of a \e{block-independent-disjoint} (BID) probabilistic database~\cite{ReS07}. In a BID, every relation is partitioned into independent blocks of mutually exclusive tuples, each associated with a probability. This model has also been studied under the terms \e{dirty database}~\cite{AndritsosFM06} and x-tuples~\cite{MaslowskiW13,ChengCX08,MoCLCY13}.  Yet, we are not aware of any positive results on inference over BIDs regarding integrity constraints. Moreover, the translation from a CIR to a BID loses the information of which attributes are certain and which are uncertain, and as aforesaid, if we allow every attribute to be uncertain then the problem is hard for every nontrivial set of FDs (Theorem~\ref{thm:all-uncertain-all-hard}).

\subparagraph*{Organization.} The remainder of the paper is organized as follows. We begin with preliminary definitions and notation (Section~\ref{sec:prelims}). We then define the CIR data model (Section~\ref{sec:cir}) and the  computational problems that we study (Section~\ref{sec:problems}). Next, we describe our analysis for the case of singleton and matching dependencies (Section~\ref{sec:single-matching}), and then the case of unary functional dependencies (Section~\ref{sec:unary}). Lastly, we give concluding remarks (Section~\ref{sec:conclusions}). Some of the proofs are omitted for lack of space, and they can be found in the Appendix. Hence, every hardness result we establish extends immediately to the most-probable-database problem over BIDs, but not vice versa.



==> trash.tex <==
To prove Part~2, we need to show hardness for $\sharpp$. Note that our reduction is \e{not} a parsimonious reduction from the problem of counting all satisfying assignments, since there is no one-to-one mapping between the satisfying truth assignments and the imputations. So, we will adapt the reduction to be a Turing reduction from a known $\sharpp$-complete variant of non-mixed satisfiability, namely the \e{1-in-3} version~\cite{creignou1993p}. In this version, we assume that we are given a 3-CNF formula, that is,
each $c_i$ is the conjunction of three literals (all positive or all negative), and the goal is to count the truth assignments wherein each $c_i$ is satisfied by precisely one literal. 

We apply the construction of Part~1, and in addition, we add the following tuples to $U$.
\begin{itemize}
    \item For each positive literal $c_i=y_1\lor y_2\lor y_3$ we add the tuples $(y_1|y_2,\false)$, $(y_1|y_3,\false)$ and $(y_2|y_3,\false)$;
    \item Analogously, for each positive literal $c_i=\neg y_1\lor \neg y_2\lor \neg y_3$ we add the tuples $(y_1|y_2,\true)$, $(y_1|y_3,\true)$ and $(y_2|y_3,\true)$.
\end{itemize}
Observe the following. An imputation requires that for each positive clause $c$, we have the tuple $(y,\true)$ for one literal in $c$, and the tuples $(y',\false)$ and $(y'',\false)$ for the other two clauses (since this is the only way to satisfy all four facts that were added for $c$). We also have the analogous situation for every negative clause. Hence, an imputation fully encodes a unique legal assignment. Similarly, each legal assignment can be likewise encoded as an imputation, where we have to choose between $y'$ and $y''$ in the tuple $(y'|y'',\false)$ defined above (or $(y'|y'',\true)$ in the case of a negative clause). Therefore, every legal satisfying assignment corresponds to $2^m$ imputations (where $m$ is the number of clauses). 

Finally, observe that every sample in the support of $U$ has the same probability: $3^{-m}\dots 2^{-3m}$. The part $3^{-m}$ corresponds to the choice of values from the reduction of Part~1, and the part of $2^{-3m}=8^{-m}$ corresponds to the choices in the new tuples added here for Part~2. It thus follows that the number legal assignments can be computed by $24^m\cdot\prob_U(\uca A\ra B)/2^m = 12^m\cdot\prob_U(\uca A\ra B)$. This completes the reduction.

\begin{lemma}\label{lemma:matching-single-tractable}
Let $X\lra Y$ be a matching constraint that includes precisely one occurrence of an uncertain attribute, and $R$ a schema that contains $X\cup Y$. A most probable imputation can be found in polynomial time.
\end{lemma}
\begin{proof}
If $X\subseteq Y$, then $X\lra Y$ is equivalent to
$\set{X\ra Y\setminus X}$ where only $Y$ contains an uncertain attribute (or otherwise both $X$ and $Y$ have include occurrences of an uncertain attribute, in contrast to the assumption of the lemma), and the tractability of this case is stated in Theorem~\ref{thm:one-FD}. The same holds if $Y\subseteq X$. So, in the remainder of the proof, we assume that
$X\not\subseteq Y$ and that $Y\not\subseteq X$. We also assume, without loss of generality (due to the symmetry between $X$ and $Y$), that $X\lra Y$ is of the form
$X'\tA\lra Y$, where $\tA$ is an uncertain attribute (as usual) and both $X'$ and $Y$ contain only certain attributes.

Let $U$ be a CIR over $R$. We will show how to find a most probable imputation of $U$ in polynomial time, assuming that one exists. We first observe that if $U$ violates $Y\ra X'$ (via its certain attributes), then $U$ is not imputable. So, we assume that $Y\ra X'$ holds. Call a maximal subset of $U$ where all tuples agree on $X'$ a \e{block}. Note that tuples from different blocks necessarily disagree on $X'$, and hence, on $Y$. 

We claim that for a sample to be an imputation of $U$, it is both necessary and sufficient to consist of an imputation for each block. In particular, to construct a most probable imputation, it suffices to find a most probable imputation for each block. Necessity is obvious, since consistency is monotonic and, in particular, preserved in each block. To see that it is sufficient, observe that two tuples from different blocks cannot violate $X\ra Y$. Indeed, they satisfy $X\ra Y$ since they disagree on $X$ (as they already disagree on $X'$), and they satisfy $Y\ra X$ since they disagree on $Y$.

So, it remains to find an imputation for a block of $U$. By definition, all tuples in the block have the same values for $X'$, and so, finding an imputation for $X\lra Y$ is the same as finding an imputation for
$\tA\lra Y$. This is done using the same least-cost-matching algorithm for $\tA\lra B$, as discussed in Section~\ref{sec:A-lra-tB}.
\end{proof}

